ATLAS measurements of the properties of jets for boosted particle searches

Measurements are presented of the properties of high transverse momentum jets, produced in proton-proton collisions at a center-of-mass energy of sqrt(s) = 7 TeV. The data correspond to an integrated luminosity of 35 pb^-1 and were collected with the ATLAS detector in 2010. Jet mass, width, eccentricity, planar flow and angularity are measured for jets reconstructed using the anti-kt algorithm with distance parameters R = 0.6 and 1.0, with transverse momentum pT > 300 GeV and pseudorapidity |eta| < 2. The measurements are compared to the expectations of Monte Carlo generators that match leading-logarithmic parton showers to leading-order, or next-to-leading-order, matrix elements. The generators describe the general features of the jets, although discrepancies are observed in some distributions.

==> Makefile <==
NOTENAME=jetprops

all:#default target makes everything
	pdflatex $(NOTENAME).tex; bibtex $(NOTENAME); pdflatex $(NOTENAME).tex;  pdflatex $(NOTENAME).tex

show:
	evince $(NOTENAME).pdf

.PHONY: clean
clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).out $(NOTENAME).blg\
	$(NOTENAME).dvi $(NOTENAME).pdf \
	$(NOTENAME).toc *~

